Good-case and Bad-case Latency of Unauthenticated Byzantine Broadcast: A Complete Categorization

This paper studies the {\em good-case latency} of {\em unauthenticated} Byzantine fault-tolerant broadcast, which measures the time it takes for all non-faulty parties to commit given a non-faulty broadcaster. For both asynchrony and synchrony, we show that $n\geq 4f$ is the tight resilience threshold that separates good-case 2 rounds and 3 rounds. For asynchronous Byzantine reliable broadcast (BRB), we also investigate the {\em bad-case latency} for all non-faulty parties to commit when the broadcaster is faulty but some non-faulty party commits. We provide matching upper and lower bounds on the resilience threshold of bad-case latency for BRB protocols with optimal good-case latency of 2 rounds. In particular, we show 2 impossibility results and propose 4 asynchronous BRB protocols.

==> CHANGELOG <==
LIPICS Style - CHANGELOG

* 10/12/2018 LIPIcs-v2019 v2.0
** New Features
*** support of metadata in PDF file (e.g. author, title, keywords) 
*** revised displaying of author-related funding acknowledgements (now displayed as part of the funding block instead of footnotes)
*** added support for cleveref package (new document option 'cleveref')
*** added support for using autoref for theorem-like environments (new document option 'autoref')
*** added new environment claim and claimproof to realize sub-proofs
*** added new environment proposition
** Bugfixes
*** fixed problems with theorem-like environments when using cleveref and autoref (see new features above)
*** switched several URL from http to https
*** fixed problems with using of ACM 2012 classification (deactivated subjclass and revised support of ccsdesc macro)
** Minor changes
*** moved ORCID symbol behind author name (according https://orcid.org/content/journal-display-guidelines)
*** added separator \and to split several affiliations
*** added warnings when package 'enumitem' or 'paralist' are loaded; they manipulate the pre-defined enumeration styles and are partly incompatible
*** preloaded package 'microtype' in style
*** revised spacings/font sizes for top matter

* 09/04/2018 LIPIcs-v2018 v1.5
** Bugfixes
*** Fixed problem with page style in case of many authors
*** Fixed aggregation of authors for ToC file

* 15/03/2018 LIPIcs-v2018 v1.4
** Bugfixes
*** Fixed enumerations
*** Fixed aggregation of authors for ToC file

* 26/02/2018 LIPIcs-v2018 v1.3
** Bugfixes
*** Fixed \hideLIPIcs
*** Fixed enumerations
*** Fixed typo
** Revised display of ORCIDs following recommendation by ORCID

* 06/02/2018 LIPIcs-v2018 v1.2
** Release of LIPIcs-v2018
*** revised author macro \author{name}{affil}{email}{orcid}{funding} 
*** added support for ORCIDs
*** switched to ACM 2012 classification system
*** added new macros for extended metadata \category, \relatedversion, \supplement, \funding, \acknowledgements
*** added warnings for missing mandatory metadata
*** added preconfigured enumeration styles based on the enumerate package
*** added option \hideLIPIcs to hide all LIPIcs related information
*** added support for line numbers
** Bugfixes
*** fixed copyright line
*** added warning when using outdated subfig package due to incompatibilities in preloaded subcaption package
*** fixed bug when using MnSymbol package
*** fixed bug in numbering in theorem-like environments used in appendix
*** fixed problems in ToC file

